Surrogate Assisted Monte Carlo Tree Search in Combinatorial Optimization

Industries frequently adjust their facilities network by opening new branches in promising areas and closing branches in areas where they expect low profits. In this paper, we examine a particular class of facility location problems. Our objective is to minimize the loss of sales resulting from the removal of several retail stores. However, estimating sales accurately is expensive and time-consuming. To overcome this challenge, we leverage Monte Carlo Tree Search (MCTS) assisted by a surrogate model that computes evaluations faster. Results suggest that MCTS supported by a fast surrogate function can generate solutions faster while maintaining a consistent solution compared to MCTS that does not benefit from the surrogate function.

==> Figures/obsolete.tex <==
"""https://graphviz.org/Gallery/directed/unix.html"""

import graphviz

u = graphviz.Digraph('unix', filename='unix.gv',
                     node_attr={ 'style': 'filled'})
u.attr(size='6,6')

u.attr('node', shape='square')
u.node('None')
u.node('Only b0')
u.node('Only b1')
u.node('Only b2')

u.attr('node', shape='circle')


u.edge('root', 'b0')
u.edge('root', 'b1')
u.edge('root', 'b2')
u.edge('root', 'None')

u.edge('b0', 'b0, b1')
u.edge('b0', 'b0, b2')
u.edge('b0', 'Only b0')


u.edge('b1', 'b1, b0')
u.edge('b1', 'b1, b2')
u.edge('b1', 'Only b1')

u.edge('b2', 'b2, b0')
u.edge('b2', 'b2, b1')
u.edge('b2', 'Only b2')

u.view()
